Silicon Dating

In order to service an ever-growing base of legacy electronics, both government and industry customers must turn to third-party brokers for components in short supply or discontinued by the original manufacturer. Sourcing equipment from a third party creates an opportunity for unscrupulous gray market suppliers to insert counterfeit devices: failed, knock-off, or otherwise inferior to the original product. This increases the supplier's profits at the expense of reduced performance/reliability of the customer's system. The most challenging class of counterfeit devices to detect is recycled counterfeits: recovered genuine devices which are re-sold as new. Such devices are difficult to detect because they typically pass performance and parametric tests but fail prematurely due to age-related wear. To address the challenge of detecting recycled devices pre-deployment, we develop Silicon Dating: a low-overhead classifier for detecting recycled integrated circuits using Static Random-Access Memory (SRAM) power-on states. Silicon Dating targets devices with no known-new record or purpose-built anti-recycling hardware. We observe that over time, software running on a device imprints its unique data patterns into SRAM through analog-domain changes; we measure the level and direction of this change through SRAM power-on state statistics. In contrast to highly symmetric power-on states produced by variation during SRAM fabrication, we show that embedded software data is generally highly asymmetric and that the degree of power-on state asymmetry imprinted by software reveals device use. Using empirical results from embedded benchmarks running on several microcontrollers, we show that Silicon Dating identifies recycled devices with 84.1% accuracy with no software-specific knowledge and with 92.0% accuracy by incorporating software knowledge---without prior device enrollment or modification.

==> Figures/SRAM_Cell.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\columnwidth]{Figures/SRAM_Cell}
  \caption{\footnotesize A typical six-transistor CMOS SRAM cell. Transistors M\textsubscript{1} and M\textsubscript{3} are NMOS devices and transistors M\textsubscript{2} and M\textsubscript{4} are PMOS devices. \hrw{Maybe combine with Figure~\ref{fig:preage_heatmap} as subfigures}}
  \label{fig:sram_cell}
\end{figure}

==> Figures/benchmarks.tex <==
\begin{table}[!t]
\footnotesize
\centering
\begin{tabular}{l c c c}
\textbf{Benchmark}            & \textbf{Code Size (B)} & \textbf{SRAM Use (B)} & \textbf{Avg. SW Bias}\\
\hline
\hline
FFT                 & 16212     & 512   & 0.3074        \\
FSM Controller      & 1542      & 468   & 0.0744        \\
FIR Filter          & 4240      & 448   & 0.3356        \\
Quicksort           & 3678      & 512   & 0.1995        \\
PID Controller      & 9714      & 384   & 0.2190        \\
String Generator    & 1024      & 447   & 0.3493        \\
\end{tabular}
\caption{\footnotesize Benchmarks that we use to test \sys{}. \hrw{Need to add stdev and some other statistics to this}}
% Source: sim_bias_analysis.py
\label{table:benchmarks}
\hrulefill
\end{table}

==> Figures/bit_selection.tex <==
\begin{figure}[ht]
  \includegraphics[width=\columnwidth]{Figures/bit_selection.png}
  \caption{\hrw{Placeholder image. Idea is to have (part of?) a software heatmap and a hardware heatmap, and show how we choose candidate aging bits from them. Maybe change software from "software bias" to "infinite-age burn-in bias"}}
  \label{fig:bit_selection}
\end{figure}

==> Figures/boards_table.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l | c c c}	
\textbf{Chip}   & MSP430G2553 & MSP432P401R & EFM32WG990F256 \\
\hline
Manufacturer        & Texas Instruments & Texas Instruments & Silicon Laboratories \\
Core                & MSP430 & ARM Cortex-M4 & ARM Cortex-M4 \\
SRAM Size (B)       & 512 & 64K & 32K \\
Aging Acceleration* & T, V & T & T \\
Dev. Board Cost (\$)& 9.99 & 19.99 & 99.99 \\
Sample Size         & 18 & 6 & x \\
\end{tabular}
\caption{\footnotesize Summary of each chip under test. *T indicates device aging can be accelerated linearly through increased temperature, V indicates device aging can be accelerated exponentially through increased voltage.}
\label{table:boards_table}
\hrulefill
\end{table}

==> Figures/bounding_aging.tex <==
\begin{figure}[ht]
  \includegraphics[width=\columnwidth]{Figures/fully_biased_sw_aware_similarity.png}
  \caption{\hrw{Replace with many boot states and the applied delta}}
  \label{fig:sw_score}
\end{figure}

\begin{figure}[ht]
  \includegraphics[width=\columnwidth]{Figures/fully_biased_sw_aware_similarity_change.png}
  \caption{\hrw{SW similarity change}}
  \label{fig:sw_score_change}
\end{figure}

\begin{figure}[ht]
  \includegraphics[width=\columnwidth]{Figures/fully_biased_sw_avg_bias_change.png}
  \caption{\hrw{Average bias change}}
  \label{fig:avg_bias_change}
\end{figure}


==> Figures/decision_table.tex <==
\begin{table}[!t]
\centering
\footnotesize
\begin{tabular}{|l|c|c|c|}
\hline
\backslashbox{\textbf{Before}}{\textbf{After}} & \makebox{\textbf{0}} & \makebox{\textbf{Weak}} & \makebox{\textbf{1}}\\
\hline
\textbf{0}          & 81.4\% & 16.1\% & 2.4\% \\
\hline
\textbf{Weak}       & 80.6\% & 12.4\% & 93.8\% \\
\hline
\textbf{1}          & 2.7\% & 14.3\% & 83.0\% \\
\hline
\end{tabular}
\caption{\footnotesize Placeholder table}
% Source: flipping_stats.py
\label{table:decision_table}
\hrulefill
\end{table}


==> Figures/many_rocs.tex <==
\begin{figure}
  \includegraphics[width=\columnwidth]{Figures/many_rocs_unaware_narrow.pdf}
  \caption{\footnotesize Software-unaware classifier ROC curves for each benchmark.}
  \label{fig:many-rocs}
\end{figure}
% Source: data from all_boards_benchmarks_two_thresholds.py plotted in many_rocs.py

==> Figures/preage_heatmap.tex <==
% Square heatmap for now - less intuitive presentation, but takes up less space

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\columnwidth]{Figures/preage_heatmap_img.pdf}
  \caption{\footnotesize MSP430G2553 SRAM startup states before aging.}
  \label{fig:preage_heatmap}
\end{figure}

==> Figures/results_table.tex <==
% % WIDE BASELINE
% \begin{table}
% \footnotesize
% \begin{tabular}{l | c c c | c c c}
%                 & \multicolumn{3}{c}{SW-Aware} & \multicolumn{3}{c}{SW-Unaware} \\	
% Benchmark       & AUC & Accuracy & J & AUC & Accuracy & J \\
% \hline
% \hline
% FFT             & 0.965 & 90.5\% & 0.809 & 0.867 & 80.5\% & 0.610 \\
% FSM             & 0.997 & 97.5\% & 0.949 & 0.984 & 93.8\% & 0.875 \\
% FIR             & 0.911 & 83.5\% & 0.670 & 0.775 & 71.0\% & 0.419 \\
% Quicksort       & 0.971 & 91.8\% & 0.835 & 0.960 & 90.1\% & 0.802 \\
% PID             & 0.952 & 88.7\% & 0.774 & 0.842 & 75.9\% & 0.517 \\
% String          & 0.758 & 69.7\% & 0.393 & 0.685 & 63.5\% & 0.269 \\
% \end{tabular}
% \caption{\footnotesize Classification performance for benchmark software. Informedness is also known as Youden's J statistic, shortened here to J.}
% % Not sure Informedness is necessary here, may remove it
% % Source: many_rocs.py with wide baseline data
% \label{table:results}
% \hrulefill
% \end{table}

% % NARROW BASELINE
% \begin{table}
% \footnotesize
% \begin{tabular}{l | c c c c | c c c c}
%                 & \multicolumn{4}{c}{SW-Aware} & \multicolumn{4}{c}{SW-Unaware} \\	
% \textbf{Benchmark}       & AUROC & TPR & FPR & Acc.    & AUROC & TPR & FPR & Acc.\\
% \hline
% \hline
% FFT             & 0.999 & 0.988 & 0.014 & 98.8\%            & 0.992 & 0.963 & 0.036 & 96.4\%    \\
% FSM             & 1.00  & 1.00  & 0.001 & 100\%             & 1.00  & 1.00  & 0.00  & 100\%     \\
% FIR             & 0.972 & 0.914 & 0.074 & 92.0\%            & 0.952 & 0.839 & 0.074 & 88.3\%    \\
% Quicksort       & 0.996 & 0.969 & 0.025 & 97.7\%            & 1.00 & 0.997 & 0.003 & 99.7\%    \\
% PID             & 0.999 & 0.986 & 0.016 & 98.7\%            & 0.987 & 0.966 & 0.082 & 94.2\%    \\
% String          & 0.879 & 0.803 & 0.239 & 81.4\%            & 0.849 & 0.795 & 0.239 & 77.8\%    \\
% \hline
% \textbf{Mean}   & 0.973 & 0.943 & 0.062 & 94.8\%            & 0.963 & 0.927 & 0.072 & 92.7\%    \\
% \end{tabular}
% \caption{\footnotesize Classification performance for benchmark software.}
% % Accuracy can be derived from TPR and FPR and I think the TPR/FPR numbers may "look" better
% % Maybe show TPR and TNR: Good high numbers
% % Source: many_rocs.py with narrow baseline data
% \label{table:results}
% \hrulefill
% \end{table}

% NARROW BASELINE WITHOUT ACCURACY NUMBER
\begin{table}
\footnotesize
\begin{tabular}{l | c c c | c c c}
                & \multicolumn{3}{c}{SW-Aware} & \multicolumn{3}{c}{SW-Unaware} \\	
\textbf{Benchmark}       & AUROC & TPR & FPR    & AUROC & TPR & FPR\\
\hline
\hline
FFT             & 0.999 & 0.988 & 0.014            & 0.992 & 0.963 & 0.036    \\
FSM             & 1.00  & 1.00  & 0.001             & 1.00  & 1.00  & 0.00     \\
FIR             & 0.972 & 0.914 & 0.074            & 0.952 & 0.839 & 0.074    \\
Quicksort       & 0.996 & 0.969 & 0.025            & 1.00 & 0.997 & 0.003    \\
PID             & 0.999 & 0.986 & 0.016            & 0.987 & 0.966 & 0.082    \\
String          & 0.879 & 0.803 & 0.239            & 0.849 & 0.795 & 0.239    \\
\hline
\textbf{Mean}   & 0.973 & 0.943 & 0.062            & 0.963 & 0.927 & 0.072    \\
\end{tabular}
\caption{\footnotesize Classification performance for benchmark software.}
% Accuracy can be derived from TPR and FPR and I think the TPR/FPR numbers may "look" better
% Maybe show TPR and TNR: Good high numbers
% Source: many_rocs.py with narrow baseline data
\label{table:results}
\hrulefill
\end{table}

==> Figures/roc_curves.tex <==
\begin{figure}
  \includegraphics[width=\columnwidth]{Figures/roc_sw_narrow.pdf}
  \caption{\footnotesize Software-aware classifier performance as a function of $T$. \hrw{Need to remove Y-index dots from these---different thresholds for each benchmark, so they don't really mean anything in the average case.}}
  \label{fig:roc_curves}
\end{figure}
% Source: data from all_boards_benchmarks_two_thresholds.py plotted in roc_curves.py

==> Figures/roc_curves_wide.tex <==
\begin{figure}[t]
  \includegraphics[width=\columnwidth]{Figures/roc_sw_wide.pdf}
  \caption{\footnotesize Classifier performance with a high-variance baseline set. \hrw{Potentially combine with other roc plot, also remove Y-index dots}}
  \label{fig:roc_curves_wide}
\end{figure}
% Source: data from all_boards_benchmarks_two_thresholds.py plotted in roc_curves.py

==> Figures/small_stripe_stats.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{l|c c c}
Region bias & \multicolumn{3}{|c}{Proportion} \\
  & 0 & Weak & 1 \\
\hline
0 & 65\% & 12\% & 23\% \\
1 & 69\% & 12\% & 19\% \\
\end{tabular}
\caption{\footnotesize Cell-bias distribution for alternately biased 512-bit regions.}
% Source: unaged_stripes.py
\label{table:small_stripe_stats}
\hrulefill
\end{table}

==> Figures/stripe_stats.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{l|c c c|c c c|c c c}
% \hline
\textbf{Cell bias}& \multicolumn{3}{c|}{Before}  & \multicolumn{3}{c|}{Aged to 0}  & \multicolumn{3}{c|}{Aged to 1}     \\
\hline
% test1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
\backslashbox{Expected}{Actual}& 0     &   Weak    &  1            & 0     &   Weak &  1                       & 0     &   Weak &  1                       \\
% \textbf{Stripe Bias}                               &       &           &               &       &        &                          &       &        &                          \\
0                               & 73\%  &   9\%     &  19\%         & 81\% & 7\% & 12\% & 68\% & 10\% & 23\% \\
1                               & 19\% & 9\% & 73\% & 26\% & 10\% & 64\% & 14\% & 8\% & 78\% \\
% \hline
\end{tabular}
\caption{\footnotesize Change in the proportion of each type of cell within each stripe. \hrw{Probably remove and replace with dots-leaving-diagonal figure}}
% Source: flipping_stats.py
\label{table:stripe_stats}
\hrulefill
\end{table}

% \begin{table}
% \centering
% \footnotesize
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Bit bias} & \textbf{New} & \textbf{Aged with} & \textbf{Aged against}   \\
% \hline
% \textbf{Strong Dominant}        & 72.60\% & 79.10\% & 66.20\%   \\
% \textbf{Strong Non-dominant}    & 18.40\% & 13.30\% & 24.10\%   \\
% \textbf{Weak}                   & 8.90\% & 7.60\% & 9.60\%      \\
% \hline
% \end{tabular}
% \caption{\footnotesize Change in the proportion of each type of cell within each stripe. \hrw{Probably remove and replace with dots-leaving-diagonal figure}}
% % Source: flipping_stats.py
% \label{table:stripe_stats}
% \hrulefill
% \end{table}

% \begin{table*}
% \centering
% \footnotesize
% \begin{tabular}{l | c c c | c c c | c c c}
%                 & \multicolumn{3}{c|}{MSP430G2553~\cite{g2553datasheet}} & \multicolumn{3}{c|}{MSP432P401R~\cite{msp432datasheet}} & \multicolumn{3}{c}{EFM32WG990F256~\cite{efm32datasheet}} \\	
% \textbf{Statistic}  & Mean & Std. Dev. & Rel. Std. Dev.           & Mean & Std. Dev & Rel. Std. Dev.     & Mean & Std. Dev & Rel. Std. Dev. \\
% \hline
% Mean bias               & 0.519  & 0.015 & 2.89\%       & xxx & xxx & xxx        & xxx & xxx & xxx \\
% Portion strong          & 88.4\% & 1.1\% & 1.24\%       & xxx & xxx & xxx        & xxx & xxx & xxx \\
% Portion weak            & 11.6\% & 1.1\% & 9.48\%       & xxx & xxx & xxx        & xxx & xxx & xxx \\
% Weak bias mean          & 0.499  & 0.016 & 3.14\%       & xxx & xxx & xxx        & xxx & xxx & xxx \\
% Weak bias std. dev.     & 0.355  & 0.0044& 1.24\%      & xxx & xxx & xxx        & xxx & xxx & xxx \\
% Portion strong 1        & 46.1\% & 1.2\% & 2.60\%       & xxx & xxx & xxx        & xxx & xxx & xxx \\
% Portion strong 0        & 42.3\% & 1.9\% & 4.49\%       & xxx & xxx & xxx        & xxx & xxx & xxx \\
% \end{tabular}
% \caption{\footnotesize SRAM power-on statistics for chips from three different microcontroller families. \hrw{RSD for first 4 not very meaningful, may remove. Also portion strong encompassed by portion strong0/strong1}}
% \label{table:new_stats}
% \hrulefill
% \end{table*}
